Single-Player and Two-Player Buttons & Scissors Games

We study the computational complexity of the Buttons \& Scissors game and obtain sharp thresholds with respect to several parameters. Specifically we show that the game is NP-complete for $C = 2$ colors but polytime solvable for $C = 1$. Similarly the game is NP-complete if every color is used by at most $F = 4$ buttons but polytime solvable for $F \leq 3$. We also consider restrictions on the board size, cut directions, and cut sizes. Finally, we introduce several natural two-player versions of the game and show that they are PSPACE-complete.

==> 1p_directions.tex <==
% !TEX root = arxiv-bands.tex

%One direction of cuts can by solved in polytime by Theorem \ref{thm:1row}.
NP-completeness for horizontal and vertical cuts and $F=7$ was proven in \cite{glsw-bsnpc-15}.
We improve this to $F=6$.

\begin{theorem}
%Buttons $\&$ Scissors with horizontal and vertical cuts and with a maximum of $F=6$ buttons per color is NP-complete.
%That is, 
$\Board{n \times n}{\infty}{6}{\dirsTwoA}{2}{B}$ is NP-complete.
\end{theorem}




==> 1p_inapprox.tex <==
% !TEX root = arxiv-bands.tex

